Improving Interpretability and Robustness for the Detection of AI-Generated Images

With growing abilities of generative models, artificial content detection becomes an increasingly important and difficult task. However, all popular approaches to this problem suffer from poor generalization across domains and generative models. In this work, we focus on the robustness of AI-generated image (AIGI) detectors. We analyze existing state-of-the-art AIGI detection methods based on frozen CLIP embeddings and show how to interpret them, shedding light on how images produced by various AI generators differ from real ones. Next we propose two ways to improve robustness: based on removing harmful components of the embedding vector and based on selecting the best performing attention heads in the image encoder model. Our methods increase the mean out-of-distribution (OOD) classification score by up to 6% for cross-model transfer. We also propose a new dataset for AIGI detection and use it in our evaluation; we believe this dataset will help boost further research. The dataset and code are provided as a supplement.

==> table_assessing_probing.tex <==
\begin{table}[!t]
    \centering\setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{\setstretch{0.95}
    \begin{tabular}{lrrrrrrrr}
        \toprule
Set of components & TreeDepth  & TopConst   & Bshift     & Tense      & SubjNum    & ObjNum     & SOMO       & CoordInv   \\
\midrule
Full              & 39.2 ± 0.3 & 73.0 ± 0.2 & 90.7 ± 0.1 & 90.3 ± 0.1 & 88.0 ± 0.1 & 85.6 ± 0.1 & 69.7 ± 0.1 & 71.6 ± 0.1 \\
On selected 49    & 26.4 ± 0.1 & 36.8 ± 0.1 & 80.8 ± 0.1 & 82.6 ± 0.1 & 73.6 ± 0.3 & 70.9 ± 0.1 & 62.5 ± 0.3 & 60.0 ± 0.2 \\
On random 49      & 25.5 ± 0.6 & 35.2 ± 0.9 & 74.4 ± 2.1 & 80.3 ± 1.9 & 73.3 ± 1.4 & 68.6 ± 1.5 & 58.6 ± 0.7 & 57.5 ± 1.0 \\
On removed 719    & 38.8 ± 0.2 & 72.3 ± 0.2 & 90.0 ± 0.0 & 90.2 ± 0.1 & 87.8 ± 0.2 & 85.2 ± 0.1 & 69.1 ± 0.3 & 71.0 ± 0.1 \\
On random 719     & 39.2 ± 0.1 & 72.6 ± 0.1 & 90.6 ± 0.1 & 90.1 ± 0.0 & 87.8 ± 0.1 & 85.5 ± 0.1 & 69.6 ± 0.2 & 71.1 ± 0.2 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Accuracy scores on probing tasks for different set of components from RoBERTa: 49 selected via greedy search and 719 remaining from greedy search. We also report the average score for randomly selected 49 and 719 components for comparison. The larger difference in the performance between the selected and random components sets on given probing task may serve as an additional signal of the importance of the tested linguistic feature for artificial text detection.}
    
    \label{tab:assessing_probing}
\end{table}

==> table_assessing_probing_v2.tex <==
\begin{table}[!t]
    \centering\setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{\setstretch{0.95}
    \begin{tabular}{lrrrrr}
        \toprule
Task               & Full       & Sel. (49) & Rand.~(49) & Rem. (719) & Rand. (719) \\
\midrule
\textbf{Syntactic} &            &                &              &                &               \\
TreeDepth          & 39.2{\scriptsize±.3} & 26.4{\scriptsize±.1}     & 25.5{\scriptsize±.6}   & 38.8{\scriptsize±.2}     & 39.2{\scriptsize±.1}    \\
TopConst           & 73.0{\scriptsize±.2} & 36.8{\scriptsize±.1}     & 35.2{\scriptsize±.9}   & 72.3{\scriptsize±.2}     & 72.6{\scriptsize±.1}    \\
Bshift             & 90.7{\scriptsize±.1} & 80.8{\scriptsize±.1}     & 74.4{\scriptsize±2.1}   & 90.0{\scriptsize±.0}     & 90.6{\scriptsize±.1}    \\
\textbf{Semantic}  &            &                &              &                &               \\
Tense              & 90.3{\scriptsize±.1} & 82.6{\scriptsize±.1}     & 80.3{\scriptsize±1.9}   & 90.2{\scriptsize±.1}     & 90.1{\scriptsize±.0}    \\
SubjNum            & 88.0{\scriptsize±.1} & 73.6{\scriptsize±.3}     & 73.3{\scriptsize±1.4}   & 87.8{\scriptsize±.2}     & 87.8{\scriptsize±.1}    \\
ObjNum             & 85.6{\scriptsize±.1} & 70.9{\scriptsize±.1}     & 68.6{\scriptsize±1.5}   & 85.2{\scriptsize±.1}     & 85.5{\scriptsize±.1}    \\
SOMO               & 69.7{\scriptsize±.1} & 62.5{\scriptsize±.3}     & 58.6{\scriptsize±.7}   & 69.1{\scriptsize±.3}     & 69.6{\scriptsize±.2}    \\
CoordInv           & 71.6{\scriptsize±.1} & 60.0{\scriptsize±.2}     & 57.5{\scriptsize±1.0}   & 71.0{\scriptsize±.1}     & 71.1{\scriptsize±.2}   \\
        \bottomrule
    \end{tabular}
    }
    \caption{Accuracy scores on probing tasks for different set of components from RoBERTa: 49 selected via greedy search and 719 remaining from greedy search. We also report the average score for randomly selected 49 and 719 components for comparison. The larger difference in the performance between the selected and random components sets on given probing task may serve as an additional signal of the importance of the tested linguistic feature for artificial text detection.}
    
    \label{tab:assessing_probing}
\end{table}

==> text_results_head_pruning_full.tex <==
\begin{table}[!t]
    \centering\setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{\setstretch{0.95}
    \begin{tabular}{lcccc}
        \toprule
             &    davinci & GPT-4 & davinci to GPT-4 & GPT-4 to davinci \\
            &    OOD & OOD              & transfer    & transfer \\
        \midrule
        Full model   & 81.3  & 64.3 & 66.4 & 70.4 \\
        \midrule
        \textbf{Pruned layer} & &  &  & \\
        \#0  & {83.2} & \textbf{80.1} & \textbf{80.0} & \textbf{83.2} \\
        \#1  & 83.4 & \underline{78.8} & \underline{74.7} & \underline{79.2} \\
        \#2  & 82.1 & \underline{78.8} & 72.7 & 77.4 \\
        \#3  & 81.8 & 82.0 & 73.6 & 78.1 \\
        \#4  & 83.4 & 79.6 & 71.6 & 76.4 \\
        \#5  & 82.2 & 78.1 & 72.9 & 75.6 \\
        \#6  &  \underline{84.0} & 76.3 & 72.3 & 74.4 \\
        \#7  & 82.8 & 75.4 & 70.1 & 74.6 \\
        \#8  & 82.8 & 72.1 & 68.5 & 73.4 \\
        \#9  & 83.2 & 73.2 & 68.7 & 71.4 \\
        \#10 & 83.1 & 71.0 & 68.1 & 72.8 \\
        \#11 & \textbf{86.6} & 68.2 & 67.3 & 71.7 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Average accuracy of artificial text detection over three domains (Wikipedia, Reddit, StackExchange) and two generating models (GPT3.5-davinci and GPT4). Detector is trained on one domain against one generator and evaluated on other domains (OOD) and on all domains against unseen generating model (transfer). Best results are given in bold, runner-ups are underlind.}
    \label{tab:text_results_pruning}
\end{table}

==> text_results_table_layers.tex <==
\begin{table}[!t]
    \centering\setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lrrrrrr}
        \toprule
        Model     &    ChatGPT             &    Cohere              & {\footnotesize davinci}                & Dolly-v2                  &  Avg                  & $q_{0.1}$\\
        \midrule
        Full      & 82.8{\scriptsize±.7}             & 80.1{\scriptsize±.6}             & 66.9{\scriptsize±.8}             & 71.4{\scriptsize±.4}             & 75.3{\scriptsize±.4}             & 51.9{\scriptsize±.3} \\
        Random    & 80.8{\scriptsize±1.5}             & 79.8{\scriptsize±.7}             & 66.1{\scriptsize±1.0}             & 74.4{\scriptsize±1.6}             & 75.3{\scriptsize±.5}             & 52.5{\scriptsize±.9} \\
        \midrule
        Layer 0   & \underline{80.3{\scriptsize±.4}} & \underline{79.2{\scriptsize±.6}} & \textbf{68.0{\scriptsize±.5}}    & \textbf{78.3{\scriptsize±.4}}    & \textbf{76.5{\scriptsize±.3}}    & \textbf{54.1{\scriptsize±.7}} \\
        Layer 1   & \underline{80.0{\scriptsize±.6}} & \textbf{81.0{\scriptsize±.7}}    & 66.4{\scriptsize±.8}             & \textbf{74.2{\scriptsize±.5}}    & 75.4{\scriptsize±.2}             & \textbf{53.6{\scriptsize±.6}} \\
        Layer 2   & \underline{77.7{\scriptsize±.4}} & 80.6{\scriptsize±.7}             & 66.3{\scriptsize±.7}             & \textbf{76.0{\scriptsize±.3}}    & 75.1{\scriptsize±.3}             & 51.8{\scriptsize±.5} \\
        Layer 3   & \underline{81.3{\scriptsize±.3}} & \textbf{80.9{\scriptsize±.6}}    & \textbf{67.7{\scriptsize±.6}}    & \textbf{75.2{\scriptsize±.3}}    & \textbf{76.3{\scriptsize±.2}}    & \textbf{54.1{\scriptsize±.9}} \\
        Layer 4   & 83.2{\scriptsize±.4}             & \textbf{81.1{\scriptsize±.4}}    & \textbf{68.0{\scriptsize±.8}}    & \textbf{73.8{\scriptsize±.2}}    & \textbf{76.5{\scriptsize±.3}}    & \textbf{53.2{\scriptsize±.3}} \\
        Layer 5   & \underline{80.9{\scriptsize±.4}} & \textbf{81.8{\scriptsize±.7}}    & 67.3{\scriptsize±.9}             & \textbf{72.4{\scriptsize±.4}}    & 75.6{\scriptsize±.2}             & \textbf{52.8{\scriptsize±.4}} \\
        Layer 6   & \underline{80.9{\scriptsize±.4}} & \textbf{80.8{\scriptsize±.8}}    & \underline{65.2{\scriptsize±.8}} & \textbf{72.3{\scriptsize±.5}}    & \underline{74.8{\scriptsize±.4}} & \textbf{52.5{\scriptsize±.3}} \\
        Layer 7   & 83.3{\scriptsize±.6}             & \textbf{81.5{\scriptsize±.7}}    & 67.7{\scriptsize±.6}             & \textbf{72.8{\scriptsize±.4}}    & \textbf{76.3{\scriptsize±.2}}    & \textbf{52.3{\scriptsize±.5}} \\
        Layer 8   & \textbf{83.8{\scriptsize±.6}}    & 80.6{\scriptsize±.8}             & \textbf{67.9{\scriptsize±.7}}    & 71.3{\scriptsize±.5}             & \textbf{75.9{\scriptsize±.3}}    & 52.0{\scriptsize±.5} \\
        Layer 9   & 82.7{\scriptsize±.7}             & \textbf{80.9{\scriptsize±.7}}    & 66.7{\scriptsize±.7}             & \textbf{72.2{\scriptsize±.6}}    & 75.6{\scriptsize±.2}             & 51.6{\scriptsize±.3} \\
        Layer 10  & \underline{81.6{\scriptsize±.7}} & 80.2{\scriptsize±.6}             & 66.6{\scriptsize±.9}             & 71.2{\scriptsize±.3}             & 74.9{\scriptsize±.4}             & 52.0{\scriptsize±.4} \\
        Layer 11  & \textbf{84.4{\scriptsize±.8}}    & \textbf{81.8{\scriptsize±.8}}    & \textbf{67.9{\scriptsize±.3}}    & \underline{70.5{\scriptsize±.6}} & \textbf{76.2{\scriptsize±.2}}    & \textbf{52.9{\scriptsize±.3}} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Mean balanced accuracy for out-of-domain classification for different pruned layers; ``Random'' shows 12 randomly pruned heads. Bold numbers show scores higher than the mean plus the standard deviation of the full model; underlined, lower than the mean minus the standard deviation.}\label{tab:text_results_layers}
\end{table}

==> text_results_table_probing.tex <==
\begin{table}[!t]
    \centering\setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{\setstretch{0.95}
    \begin{tabular}{lrrrrrr}
        \toprule
        Model     &    ChatGPT             &    Cohere              & {\footnotesize davinci}                & Dolly-v2                  &  Avg                  & $q_{0.1}$\\
        \midrule
        Full      & 82.8{\scriptsize±.7}  & 80.1{\scriptsize±.6}  & 66.9{\scriptsize±.8} & 71.4{\scriptsize±.4}  & 75.3{\scriptsize±.4} & 51.9{\scriptsize±.3} \\
        Random    & 78.1{\scriptsize±1.7} & 73.7{\scriptsize±2.0}	 & 64.5{\scriptsize±1.5}  & 66.3{\scriptsize±2.4}  & 70.7{\scriptsize±1.3} & 53.0{\scriptsize±1.8} \\
        \midrule
        \textbf{Syntactic} & & & & & & \\
        TreeDepth & 83.0{\scriptsize±.9}            & \textbf{81.4{\scriptsize±.6}}   & \textbf{69.9{\scriptsize±.5}} & \underline{68.7{\scriptsize±.5}} & \textbf{75.8{\scriptsize±.4}}      & \textbf{55.9{\scriptsize±.7}} \\
        TopConst  & \underline{79.7{\scriptsize±.6}} & \underline{70.8{\scriptsize±.5}} & 67.2{\scriptsize±.3}          & \underline{67.1{\scriptsize±.3}} & \underline{71.2{\scriptsize±.2}} & \textbf{55.3{\scriptsize±.7}} \\
        Bshift    & \underline{80.4{\scriptsize±.4}} & \underline{78.5{\scriptsize±.8}} & \textbf{68.2{\scriptsize±.3}} & \underline{70.8{\scriptsize±.6}} & \underline{74.5{\scriptsize±.3}} & \textbf{55.0{\scriptsize±.9}} \\
        \textbf{Semantic} & & & & & & \\
        Tence     & \underline{80.0{\scriptsize±.7}} & \underline{75.9{\scriptsize±.6}} & 66.6{\scriptsize±.6}          & \underline{66.4{\scriptsize±.4}} & \underline{72.2{\scriptsize±.2}} & \textbf{53.2{\scriptsize±.7}}  \\
        SubjNum   & 83.0{\scriptsize±.6}            & \underline{75.6{\scriptsize±.7}} & \textbf{68.8{\scriptsize±.4}} & \underline{69.9{\scriptsize±.2}} & \underline{74.3{\scriptsize±.3}} & \textbf{59.0{\scriptsize±.9}}  \\
        ObjNum    & \underline{78.8{\scriptsize±.7}} & \underline{76.9{\scriptsize±.5}} & 67.4{\scriptsize±.4}          & \underline{69.0{\scriptsize±.6}} & \underline{73.0{\scriptsize±.4}} & \textbf{53.5{\scriptsize±.5}}  \\
        SOMO      & \underline{80.8{\scriptsize±.3}} & \underline{76.9{\scriptsize±.5}} & 67.6{\scriptsize±.5}          & \underline{66.9{\scriptsize±.7}} & \underline{73.0{\scriptsize±.3}} & \textbf{53.4{\scriptsize±.4}}  \\
        CoordInv  & \underline{76.5{\scriptsize±.3}} & \underline{74.7{\scriptsize±.5}} & 67.3{\scriptsize±.6}          & \underline{64.6{\scriptsize±.5}} & \underline{70.8{\scriptsize±.3}} & \textbf{52.9{\scriptsize±.5}}  \\
        \bottomrule
    \end{tabular}
    }
    \caption{Mean balanced accuracy for out-of-domain classification for 100 significant features for different probing tasks. ``Random'' shows 100 randomly selected embedding components. Bold numbers show scores higher than the mean plus the standard deviation of the full model; underlined, lower than the mean minus the standard deviation.}
    \label{tab:text_results_probing}
\end{table}

==> text_results_table_residuals.tex <==
\begin{table}[!t]
    \centering
    \begin{tabular}{lrrrr}
        \toprule
        Model     &    ChatGPT   &    cohere    & davinci      & dolly  \\
        \midrule
        LogReg    & 82.8 ± 0.7 & 80.1 ± 0.6 & 66.9 ± 0.8 & 71.4 ± 0.4   \\
        Residuals & 73.4 ± 0.2 & 71.7 ± 0.2 & 67.9 ± 0.2 & 67.1 ± 0.2  \\
        \bottomrule
    \end{tabular}
    \caption{Mean balanced accuracy across out-of-domain AI-written text classification for Logistic Regression baseline and Residuals}
    \label{tab:text_results_general}
\end{table}
